When Do Voters Stop Caring? Estimating the Shape of Voter Utility Function

In this paper, we address a longstanding puzzle over the functional form that better approximates voter's political utility. Though it has become the norm in the literature to represent the voters' political utility with concave loss functions, for decades scholars have underscored this assumption's potential shortcomings. Yet there exists little to no evidence to support one functional form assumption over another. We fill this gap by first identifying electoral settings where the different functional forms generate divergent predictions about voter behavior. Then, we assess which functional form better matches observed voter and abstention behavior using Cast Vote Record (CVR) data that captures the anonymized ballots of millions of voters in the 2020 U.S. general election. Our findings indicate that concave loss functions fail to predict voting and abstention behavior and it is the reverse S-shaped loss functions, such as the Gaussian function, that better match the observed voter behavior.

==> figures/fig_uni_dim_delta.tex <==
\begin{tikzpicture}
    \coordinate (cD) at (0,0);
    \coordinate (x_i) at (2,0);
    \coordinate (x_{i'}) at (4,0);
    \coordinate (cR) at (6,0);
    \draw (cD) -- (cR);

     \foreach \point in {cD,{x_i},{x_{i'}},cR}
        \fill (\point) circle (2pt) node[below] {\point};
    
    \draw[->, thick] (2,0.2) arc (180:0:1) node[midway, above] {$\Delta{x_i}$};
\end{tikzpicture}



==> tables/ballot_dum_ideo_rolloff.tex <==
\begin{table}[!h]

\caption{Ideology and Roll-off in LA County Dem v. Dem House Races, 2020}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lcccccc}
\toprule
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule

Extremely Liberal & \num{-0.334}*** & \num{-0.151}*** & \num{-0.057}*** & \num{-0.021}*** & \num{-0.005}*** & \\
 & (\num{0.002}) & (\num{0.002}) & (\num{0.002}) & (\num{0.002}) & (\num{0.001}) & \\
Very Liberal & \num{-0.329}*** & \num{-0.147}*** & \num{-0.053}*** & \num{-0.016}*** &  & \num{0.005}***\\
 & (\num{0.002}) & (\num{0.002}) & (\num{0.002}) & (\num{0.002}) &  & (\num{0.001})\\
Liberal & \num{-0.314}*** & \num{-0.131}*** & \num{-0.037}*** &  & \num{0.016}*** & \num{0.021}***\\
 & (\num{0.002}) & (\num{0.003}) & (\num{0.002}) &  & (\num{0.002}) & (\num{0.002})\\
Conservative & \num{-0.277}*** & \num{-0.094}*** &  & \num{0.037}*** & \num{0.053}*** & \num{0.057}***\\
 & (\num{0.003}) & (\num{0.003}) &  & (\num{0.002}) & (\num{0.002}) & (\num{0.002})\\
Very Conservative & \num{-0.183}*** &  & \num{0.094}*** & \num{0.131}*** & \num{0.147}*** & \num{0.151}***\\
 & (\num{0.003}) &  & (\num{0.003}) & (\num{0.003}) & (\num{0.002}) & (\num{0.002})\\
Extremely Conservative &  & \num{0.183}*** & \num{0.277}*** & \num{0.314}*** & \num{0.329}*** & \num{0.334}***\\
 &  & (\num{0.003}) & (\num{0.003}) & (\num{0.002}) & (\num{0.002}) & (\num{0.002})\\
\midrule
No. of Observations & \num{296846} & \num{296846} & \num{296846} & \num{296846} & \num{296846} & \num{296846}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textit{Note: } Robust standard errors in parentheses.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}+ p $<$ 0.1, * p $<$ 0.05, ** p $<$ 0.01, *** p $<$ 0.001}\\
\end{tabular}
\end{table}


==> tables/ballot_ideo_rolloff.tex <==
\begin{table}[!h]

\caption{Ideology and Roll-off in LA County Top-2 House Races 2020}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lcc}
\toprule
  & All voters & Trump voters\\
\midrule
Ideology & \num{0.130}*** & \num{0.140}***\\
 & (\num{0.003}) & (\num{0.008})\\
\midrule
No. of Observations & \num{408602} & \num{105437}\\
\bottomrule
\multicolumn{3}{l}{\rule{0pt}{1em}\textit{Note: } Robust standard errors in parentheses.}\\
\multicolumn{3}{l}{\rule{0pt}{1em}+ p $<$ 0.1, * p $<$ 0.05, ** p $<$ 0.01, *** p $<$ 0.001}\\
\end{tabular}
\end{table}


==> tables/cand_ideo_cross29.tex <==
\begin{table}

\caption{Candidate Choice by Ideology Score for 
                          CA's 29th Congressional District 2020 Election}
\centering
\begin{tabular}[t]{l|r|r}
\hline
  & Angelica Maria Duenas (D, -2.867) & Tony Cardenas (D, -0.635)\\
\hline
Extremely liberal & 4759 & 4943\\
\hline
Very Liberal & 5604 & 5836\\
\hline
Liberal & 3365 & 4906\\
\hline
Conservative & 2481 & 3748\\
\hline
Very Conservative & 1896 & 3003\\
\hline
Extremely Conservative & 3141 & 4097\\
\hline
\end{tabular}
\end{table}


==> tables/cand_ideo_cross34.tex <==
\begin{table}

\caption{Candidate Choice by Ideology Score, 
                          CA's 34th Congressional District election 2020}
\centering
\begin{tabular}[t]{l|r|r}
\hline
  & David Kim (D, ) & Jimmy Gomez (D, -1.217)\\
\hline
Extremely liberal & 4393 & 5709\\
\hline
Very Liberal & 5963 & 5959\\
\hline
Liberal & 2884 & 3787\\
\hline
Conservative & 2072 & 2495\\
\hline
Very Conservative & 1594 & 1501\\
\hline
Extremely Conservative & 2272 & 1532\\
\hline
\end{tabular}
\end{table}


==> tables/cand_ideo_cross38.tex <==
\begin{table}

\caption{Candidate Choice by Ideology Score, 
                          CA's 38th Congressional District election 2020}
\centering
\begin{tabular}[t]{l|r|r}
\hline
  & Linda T. Sanchez (D, -0.831) & Michael Tolar(D, )\\
\hline
Extremely liberal & 14661 & 3298\\
\hline
Very Liberal & 16846 & 4622\\
\hline
Liberal & 13916 & 3616\\
\hline
Conservative & 11169 & 3557\\
\hline
Very Conservative & 8918 & 4507\\
\hline
Extremely Conservative & 11848 & 11179\\
\hline
\end{tabular}
\end{table}


==> tables/cand_ideo_cross44.tex <==
\begin{table}

\caption{Candidate Choice by Ideology Score, 
                          CA's 44th Congressional District election 2020}
\centering
\begin{tabular}[t]{l|r|r}
\hline
  & Analilia Joya (D, ) & Nanette Diaz Barragan(D, -1.26)\\
\hline
Extremely liberal & 3923 & 7153\\
\hline
Very Liberal & 4938 & 8235\\
\hline
Liberal & 3994 & 6154\\
\hline
Conservative & 2802 & 4112\\
\hline
Very Conservative & 2078 & 2778\\
\hline
Extremely Conservative & 3008 & 2895\\
\hline
\end{tabular}
\end{table}


==> tables/corr_indiff_table_ideo_fe.tex <==
\begin{table}[!h]
\centering\centering
\caption{}
\centering
\fontsize{11}{13}\selectfont
\begin{tabular}[t]{lc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{ } & \multicolumn{1}{c}{Abstention} \\
\cmidrule(l{3pt}r{3pt}){4-4}
  & (1)\\
\midrule
Vote Predictability & \num{-0.011}*\\
 & (\num{0.004})\\
\midrule
No. of Observations & \num{810}\\
Voter Group Fixed Effects & Yes\\
\bottomrule
\multicolumn{2}{l}{\rule{0pt}{1em}\textit{Note: } Standard errors in parentheses.}\\
\multicolumn{2}{l}{\rule{0pt}{1em}* p $<$ 0.01}\\
\end{tabular}
\end{table}


==> tables/func_form_properties_C1.tex <==
\begin{table}
\caption{Case 1 Functional Form Properties and Predictions}
\resizebox{\textwidth}{!}{ 
\fontsize{20}{28}\selectfont
\begin{tabular}{|c|l|c|c|l|} 
\hline 
\textbf{\Large Predictions}   &\textbf{\Large \textit{Functional Form}} 
& 

\multicolumn{2}{|c|}{\raisebox{-3mm}{\textbf{\Large \makecell{Reverse Sigmoid \\ Probabilistic Voting}}}} & 
\raisebox{-0.02mm}{\textbf{ \Large \makecell{Empirical Predictions}}}\\\hline 
\tikzvotingderivativesone  &\raisebox{20mm}{\Large{\makecell{Linear \\  Quadratic}}}& 
\multicolumn{2}{|c|}{} & 
\raisebox{20mm}{\Large{\makecell{Equal shift in \\ Democratic party support \\ across all \emph{Voter Group}s}}} \\ \hline 
\tikzvotingderivativestwo  &\raisebox{20mm}{\Large{\makecell{Convex \\  High Concave}}}& 
\multicolumn{2}{|c|}{} & 
\raisebox{20mm}{\Large{\makecell{Biggest shift in \\ party support occurs \\ at the extreme ends \\ of  \emph{Voter Group}}}}\\ \hline
\tikzvotingderivativesthree  &\raisebox{20mm}{\Large{\makecell{Low concave }}} 
& 
\multicolumn{2}{|c|}{} & \raisebox{20mm}{\Large{\makecell{Greatest shift in \\ Democratic party support  \\ amongst `Moderate' voters}}}\\ \hline
\tikzvotingderivativesfour  &\raisebox{20mm}{\Large{Reverse S-shaped}} & 
\multicolumn{2}{|c|}{\raisebox{20mm}{\Large{All}}} & 
\raisebox{20mm}{\Large{\makecell{Greatest shift in \\ Democratic party support \\ amongst `Moderate' voters}}} \\
\hline
\end{tabular}}
\label{table_func_forms_C1}
\end{table}







==> tables/func_form_properties_C1_multi.tex <==
\begin{table}
\caption{Case 1 Functional Form Properties and Predictions}
\resizebox{\textwidth}{!}{ 
\fontsize{20}{28}\selectfont
\begin{tabular}{|c|c c|c|c|l|} 
\hline 
\textbf{\Large Model Predictions} & 
\multicolumn{2}{c|}{\textbf{\Large Linear Probabilistic Voting}} & 

\multicolumn{2}{c|}{\raisebox{-3mm}{\textbf{\Large \makecell{Reverse Sigmoid \\ Probabilistic Voting}}}} & 
\raisebox{-0.02mm}{\textbf{ \Large \makecell{Empirical Predictions}}}\\ & 
\textbf{\Large \textit{Uni-dimensional}} & 
\textbf{\Large \textit{Multi-dimensional}} & 
\multicolumn{2}{c|}{} &\\\hline 
\tikzvotingderivativesone &
\raisebox{20mm}{\Large{\makecell{Linear, \\ Quadratic}}} & 
\raisebox{20mm}{\Large{Quadratic}} & 
\multicolumn{2}{c|}{} & 
\raisebox{20mm}{\Large{\makecell{Equal shift in \\ Democratic party support \\ across all \emph{Voter Group}s}}} \\ \hline 
\tikzvotingderivativestwo & 
\raisebox{20mm}{\Large{\makecell{Convex, \\ High Concave}}} & 
\raisebox{20mm}{\Large{\makecell{Linear, Convex, \\ High/Low Concave}}} & 
\multicolumn{2}{c|}{} & 
\raisebox{20mm}{\Large{\makecell{Biggest shift in \\ party support occurs \\ at the extreme ends \\ of  \emph{Voter Group}}}}\\ \hline
\tikzvotingderivativesthree & 
\raisebox{20mm}{\Large{\makecell{Low concave \\ ($\beta\in(1,2)$)}}} & & 
\multicolumn{2}{c|}{} & \raisebox{20mm}{\Large{\makecell{Greatest shift in \\ Democratic party support  \\ amongst `Moderate' voters}}}\\ \hline
\tikzvotingderivativesfour & 
\raisebox{20mm}{\Large{Reverse Sigmoid}} & 
\raisebox{20mm}{\Large{Reverse Sigmoid}} & 
\multicolumn{2}{c|}{\raisebox{20mm}{\Large{All}}} & 
\raisebox{20mm}{\Large{\makecell{Greatest shift in \\ Democratic party support \\ amongst `Moderate' voters}}} \\
\hline
\end{tabular}}
\label{table_func_forms_C1}
\end{table}







==> tables/func_form_properties_C2_multi.tex <==
\begin{table}
\caption{Case 2 Functional Form Properties and Predictions}
\resizebox{\textwidth}{!}{ 
\fontsize{10}{12}\selectfont
     \begin{tabular}{|c|c|c|c|l|} 
        \hline 
        \raisebox{-3mm}{\textbf{\normalsize Predictions over}:}&
        \raisebox{-3mm}{\textbf{\normalsize Predictions over}:}& 
        & & 
        \raisebox{-9mm}{{ \normalsize \makecell{\textbf{Empirical} \\ \textbf{Predictions} \\ (As min. distance to \\ candidates increases)}}}\\
        \raisebox{9mm}{$\mathbf{-|u_i(c_{D_1})-u_i(c_{D_2})|}$} & 
        \raisebox{7mm}{$\mathbf{\dfrac{-|u_i(c_{D_1})-u_i(c_{D_2})|}{\Delta d_n}}$} & 
        \raisebox{10mm}{\textbf{\normalsize Uni-dimensional}} &
        \raisebox{10mm}{\textbf{\normalsize Multi-dimensional}} &\\
        \hline 
         \tikzindiffoverKone &
        \raisebox{14mm}{$0$} &
        \raisebox{14mm}{Linear} &
        \raisebox{14mm}{Quadratic}  &\raisebox{14mm}{\makecell{Voter indifference \\ stays the same}}\\ 
        \hline 
        \tikzindiffoverKtwo &
        \raisebox{14mm}{$>0$} &
        \raisebox{14mm}{Concave} &
        \raisebox{14mm}{High Concave}  &\raisebox{14mm}{\makecell{Voters becomes less \\ indifferent}}\\ 
        \hline
        \tikzindiffoverKthree &
        \raisebox{14mm}{$<0$} &
        \raisebox{14mm}{Convex} &
        \raisebox{14mm}{Linear, Low Concave} &\raisebox{14mm}{\makecell{Voter becomes more \\ indifferent}}\\
        \hline
        \tikzindiffoverKfour &
        \raisebox{14mm}{$>0$ and $<0$} &
        \raisebox{14mm}{Reverse Sigmoid} &
        \raisebox{14mm}{Reverse Sigmoid}  &\raisebox{14mm}{\makecell{Voter becomes less \\indifferent below a \\minimum distance\\ threshold, and more \\ indifferent above \\ the threshold}}\\
        \hline
    \end{tabular}}
\label{func_form_properties_C2}
\end{table}


==> tables/n/CA/N-nonabs-sandiego-stballot.tex <==
1,627,753


==> tables/n/CA/N-nonfrag-complete-with-office-stballot.tex <==
4,044,524



==> tables/n/CA/N-nonfrag_NONABS-sandiego-stballot.tex <==
1,372,302


==> tables/n/CA/N-nonfrag_NONABS-stballot.tex <==
6,050,053


==> tables/n/CO/N-nonfrag_NONABS-stballot.tex <==
2,757,930


==> tables/perc_down.tex <==
\begin{table}[!h]
\centering
\caption{Proportion of Voter Group Subgroup Pairs with Downward Change in Democratic Support}
\centering
\begin{tabular}[t]{lr}
\toprule
Proposition & Proportion\\
\midrule
Amendment 76 & 1.000\\
Amendment B & 0.926\\
Proposition 113 & 1.000\\
Proposition 114 & 0.992\\
Proposition 115 & 1.000\\
Proposition 116 & 1.000\\
Proposition 117 & 0.852\\
Proposition 118 & 1.000\\
Proposition EE & 0.988\\
\bottomrule
\end{tabular}
\end{table}


==> tables/polar.tex <==
\begin{table}[!h]
\centering\centering
\caption{Race Polarization and Roll-off in California 2020}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Linear Piecewise} & \multicolumn{1}{c}{Quadratic} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-4}
  & (1) & (2) & (3)\\
\midrule
Race Polarization & \num{-0.826}* & \num{0.275}* & \num{-8.228}*\\
 & (\num{0.094}) & (\num{0.007}) & (\num{0.148})\\
 & & &\\
Race Polarization^{2} &  &  & \num{4.474}*\\
 &  &  & (\num{0.081})\\
\midrule
No. of Observations & \num{169004} & \num{1718859} & \num{1887863}\\
Voter Fixed Effects & Yes & Yes & Yes\\
\bottomrule
\multicolumn{4}{l}{\rule{0pt}{1em}\textit{Note: } Standard errors in parentheses.}\\
\multicolumn{4}{l}{\rule{0pt}{1em}* p $<$ 0.01}\\
\end{tabular}
\label{table_polar}
\end{table}


==> tables/polar_co.tex <==
\begin{table}[!h]
\centering\centering
\caption{US House Race Polarization and Roll-off in Colorado 2020}
\centering
\fontsize{10}{11}\selectfont
\begin{tabular}[t]{lcclc}
\toprule
  & \multicolumn{2}{c}{Linear Piecewise}&&Quadratic\\
 & (1)&  (2) &&(3)\\
 \midrule
Race Polarization & \num{-0.308}* & \num{0.234}*  && \num{-2.189}*\\
 & (\num{0.046}) & (\num{0.012})  && (\num{0.286})\\
 & &  &&\\
Polarization^{2}&  &   && \num{1.290}*\\
 &  &   && (\num{0.155})\\
\midrule
No. of Observations & \num{610172} & \num{716379}  && \num{1326551}\\
 Voter Fixed Effects& Yes& Yes& &Yes\\
\bottomrule
\multicolumn{4}{l}{\rule{0pt}{1em}Standard errors in parentheses.} &\\
\multicolumn{4}{l}{\rule{0pt}{1em}* p $<$ 0.01} &\\
\end{tabular}
\label{table_polar_co}
\end{table}


==> tables/polar_mod_table.tex <==

\begin{table}
\centering
\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{
\begin{tabular}{>{}l|ccccl}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Models} \\
\cmidrule(l{3pt}r{3pt}){2-5}
model & term & estimate & std.error & statistic & p.value\\
\midrule
\textbf{\cellcolor{gray!10}{mNpolar_mod}} & \cellcolor{gray!10}{(Intercept)} & \cellcolor{gray!10}{0.1805129} & \cellcolor{gray!10}{0.0089085} & \cellcolor{gray!10}{20.2630322} & \cellcolor{gray!10}{0.0000000}\\
\addlinespace[0.3em]
\multicolumn{6}{l}{\textbf{Polar Interaction}}\\
\hspace{1em}\textbf{mNpolar_mod} & polar & -0.1688029 & 0.0097132 & -17.3787833 & 0.0000000\\
\hspace{1em}\textbf{\cellcolor{gray!10}{mNpolar_Nmod}} & \cellcolor{gray!10}{(Intercept)} & \cellcolor{gray!10}{0.1591982} & \cellcolor{gray!10}{0.0022316} & \cellcolor{gray!10}{71.3383780} & \cellcolor{gray!10}{0.0000000}\\
\textbf{mNpolar_Nmod} & polar & -0.1515606 & 0.0024348 & -62.2466776 & 0.0000000\\
\textbf{\cellcolor{gray!10}{mpolar_Nmod}} & \cellcolor{gray!10}{(Intercept)} & \cellcolor{gray!10}{0.0405849} & \cellcolor{gray!10}{0.0307462} & \cellcolor{gray!10}{1.3199971} & \cellcolor{gray!10}{0.1868362}\\
\textbf{mpolar_Nmod} & polar & -0.0285032 & 0.0318325 & -0.8954132 & 0.3705664\\
\textbf{\cellcolor{gray!10}{mpolar_mod}} & \cellcolor{gray!10}{(Intercept)} & \cellcolor{gray!10}{-0.3424162} & \cellcolor{gray!10}{0.1316529} & \cellcolor{gray!10}{-2.6009007} & \cellcolor{gray!10}{0.0092992}\\
\textbf{mpolar_mod} & polar & 0.3763958 & 0.1363057 & 2.7614090 & 0.0057562\\
\bottomrule
\multicolumn{6}{l}{\rule{0pt}{1em}Note: Robust standard errors in parentheses.}\\
\multicolumn{6}{l}{\rule{0pt}{1em}\textsuperscript{*} + p < 0.1, * p < 0.05, ** p < 0.01, *** p < 0.001}\\
\end{tabular}}
\end{table}


==> tables/polar_predict.tex <==
\begin{table}[!h]
\centering\centering
\caption{Race Polarization and Vote Predictability in California 2020}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Linear Piecewise} & \multicolumn{1}{c}{Quadratic} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-4}
  & (1) & (2) & (3)\\
\midrule
Race Polarization & \num{2.101}* & \num{-4.493}* & \num{48.389}*\\
 & (\num{0.011}) & (\num{0.004}) & (\num{0.101})\\
Race Polarization^{2} &  &  & \num{-27.994}*\\
 &  &  & (\num{0.054})\\
\midrule
No. of Observations & \num{169053} & \num{1719518} & \num{1888571}\\
Voter Fixed Effects & No & No & No\\
\bottomrule
\multicolumn{4}{l}{\rule{0pt}{1em}\textit{Note: } Standard errors in parentheses.}\\
\multicolumn{4}{l}{\rule{0pt}{1em}* p $<$ 0.01}\\
\end{tabular}
\label{table_polar_pred}
\end{table}


==> tables/polar_predict_co.tex <==
\begin{table}[!h]
\centering\centering
\caption{US House Race Polarization and Vote Predictability in Colorado 2020}
\centering
\fontsize{10}{11}\selectfont
\begin{tabular}[t]{lcclc}
\toprule
  & \multicolumn{2}{c}{Linear Piecewise}&& Quadratic\\
   & (1) &  (2)  && (3)\\
\midrule
Race Polarization & \num{15.772}* & \num{-0.842}*  && \num{57.710}*\\
 & (\num{0.000}) & (\num{0.010})  && (\num{0.243})\\
 & & & &\\
Race Polarization^{2} &  &   && \num{-30.493}*\\
 &  &   && (\num{0.131})\\
\midrule
No. of Observations & \num{610172} & \num{716379}  && \num{1326551}\\
\bottomrule
\multicolumn{4}{l}{\rule{0pt}{1em}
Standard errors in parentheses.} &\\
\multicolumn{4}{l}{\rule{0pt}{1em}* p $<$ 0.01} &\\
\end{tabular}
\label{table_polar_pred_co}
\end{table}


==> tables/prop_14_summary.tex <==
\setlength{\LTpost}{0mm}
\begin{longtable}{lccc}
\toprule
\textbf{Characteristic} & \textbf{Beta} & \textbf{95\% CI}\textsuperscript{\textit{1}} & \textbf{p-value} \\ 
\midrule\addlinespace[2.5pt]
prop\_14 & 0.05 & 0.04, 0.05 & <0.001 \\ 
prop\_14 & 0.06 & 0.06, 0.07 & <0.001 \\ 
prop\_14 & 0.08 & 0.08, 0.08 & <0.001 \\ 
prop\_14 & 0.07 & 0.07, 0.07 & <0.001 \\ 
prop\_14 & 0.04 & 0.04, 0.04 & <0.001 \\ 
prop\_14 & 0.02 & 0.02, 0.03 & <0.001 \\ 
prop\_14 & 0.01 & 0.01, 0.01 & <0.001 \\ 
prop\_14 & 0.01 & 0.01, 0.01 & <0.001 \\ 
prop\_14 & 0.01 & 0.01, 0.01 & <0.001 \\ 
prop\_14 & 0.01 & 0.01, 0.01 & <0.001 \\ 
prop\_14 & 0.01 & 0.01, 0.01 & <0.001 \\ 
\bottomrule
\end{longtable}
\begin{minipage}{\linewidth}
\textsuperscript{\textit{1}}CI = Confidence Interval\\
\end{minipage}



==> tables/voting_ideo_rsquared.tex <==
\begin{table}[H] 
\centering 
\caption{\bf R-Squares From Regressions of Ideology on Vote Choice} 
\label{cand_ideo_rsquare} 
\scalebox{.85}{ 
\begin{tabular}{l l c c c r} 
\toprule\toprule 
        &        & 1-Dim  & Items      & Vote    &      \\ 
State   & Office & Score  & Separately & Vectors & Obs. \\ 
\midrule 
CA & US President   & 0.488 & 0.487 & 0.520 &    8,243,971 \\ 
CA & US House       & 0.500 & 0.497 & 0.529 &    7,194,192 \\ 
CA & State Senate   & 0.519 & 0.517 & 0.547 &    3,401,692 \\ 
CA & State Assembly & 0.490 & 0.489 & 0.517 &    6,116,158 \\ [.05in] 
CO & US President   & 0.453 & 0.494 & 0.511 &    2,992,966 \\ 
CO & US Senate      & 0.448 & 0.492 & 0.505 &    2,988,069 \\ 
CO & US House       & 0.549 & 0.603 & 0.616 &    2,952,210 \\ 
CO & State Senate   & 0.554 & 0.609 & 0.627 &    1,353,087 \\ 
CO & State House    & 0.553 & 0.607 & 0.621 &    2,574,580 \\  [.05in] 
\bottomrule 
\end{tabular}
} 
\end{table} 

